Vision-based GNSS-Free Localization for UAVs in the Wild

Considering the accelerated development of Unmanned Aerial Vehicles (UAVs) applications in both industrial and research scenarios, there is an increasing need for localizing these aerial systems in non-urban environments, using GNSS-Free, vision-based methods. Our paper proposes a vision-based localization algorithm that utilizes deep features to compute geographical coordinates of a UAV flying in the wild. The method is based on matching salient features of RGB photographs captured by the drone camera and sections of a pre-built map consisting of georeferenced open-source satellite images. Experimental results prove that vision-based localization has comparable accuracy with traditional GNSS-based methods, which serve as ground truth. Compared to state-of-the-art Visual Odometry (VO) approaches, our solution is designed for long-distance, high-altitude UAV flights. Code and datasets are available at https://github.com/TIERS/wildnav.

==> algs/offboard.tex <==
\begin{algorithm}[t]
	\caption{Offboard control }
	\label{alg:offboard_algorithm}
	\KwIn{ \\
	    \hspace{1em} Arming command \\
	    \hspace{1em} 3D waypoint list in the form of local (x,y,z) coordinates \\
	}
	\KwOut{\\
	    \hspace{1em} Periodic ROS 2 messages containing intermediary local coordinates  \\
	}
	 \BlankLine
	 \While{$True$}{
	 
    	 \Switch{STATE}{
                \Case{ARMED}{
                    enable\_offboard\_mode$\left(\right)$
                }
                \Case{TAKE\_OFF}{
                    publish\_takeoff\_command$\left(\right)$
                }
                 \Case{START\_MISSION}{
                   \For {$waypoint=1,N$}{
                        compute\_path$\left(currentWaypoint, nextWaypoint, speedFactor\right)$
                   }
                }
                \Case{END\_MISSION}{
                    publish\_land\_command$\left(\right)$
                }
            }        
        publish\_trajectory\_waypoint$\left(x,y,z\right)$
    }
\end{algorithm}


==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}
